Learning Named Entity Tagger using Domain-Specific Dictionary

Recent advances in deep neural models allow us to build reliable named entity recognition (NER) systems without handcrafting features. However, such methods require large amounts of manually-labeled training data. There have been efforts on replacing human annotations with distant supervision (in conjunction with external dictionaries), but the generated noisy labels pose significant challenges on learning effective neural models. Here we propose two neural models to suit noisy distant supervision from the dictionary. First, under the traditional sequence labeling framework, we propose a revised fuzzy CRF layer to handle tokens with multiple possible labels. After identifying the nature of noisy labels in distant supervision, we go beyond the traditional framework and propose a novel, more effective neural model AutoNER with a new Tie or Break scheme. In addition, we discuss how to refine distant supervision for better NER performance. Extensive experiments on three benchmark datasets demonstrate that AutoNER achieves the best performance when only using dictionaries with no additional human effort, and delivers competitive results with state-of-the-art supervised benchmarks.

==> 00-abs.tex <==
%!Tex Root = 0_main.tex

Recent advances in deep neural models allow us to build reliable named entity recognition (NER) systems without handcrafting features.
However, such methods require large amounts of human-annotated training data.
Imperfect labeled data generated by distant supervision has been found useful in a variety of tasks but remains to be further explored for NER.
In this study, we propose AutoNER, an automated framework for building NER systems with domain-specific dictionary only.
Specifically, we propose to tailor the dictionary based on the corpus and introduce unknown-typed quality phrases to improve the label effectiveness; 
In order to better leverage the unknown-typed phrases, we propose a new ``Tie or Break'' tag scheme and a novel neural architecture to make independent predictions.
Experiments on two biomedical datasets demonstrate that, without any human annotation, AutoNER achieves competitive results with state-of-the-art supervised benchmarks.
